I2C-GRPO: Insight Importance Checklist for Reinforcement Learning in a Multi-Agent DDoS Alert Triage Workflow

Large language model (LLM) agents are increasingly used for investigative tasks over incomplete evidence, such as cybersecurity alert triage, but reinforcement learning (RL) for such tasks is difficult: intermediate steps have no verifiable labels, rollouts are costly, and outcome rewards are sparse. We propose Insight Importance Checklist (I2C)-GRPO, a checklist reward for intermediate investigation steps. For each decision point, a panel of expert LLMs proposes investigative actions, their atomic forensic insights are extracted, and a separate three-model ranker panel orders the insights by importance. A reward model checks which ranked insights a candidate action targets and returns their consensus-weighted coverage. Because actions are scored without being executed, the reward is a proxy for expected investigative value, and training reduces to a one-step contextual bandit over fixed investigation prefixes. From a soft-computing perspective, the reward is an additive fuzzy measure whose rank-exponent weights act as an ordered weighted averaging (OWA)-type operator; one exponent sets its orness, i.e., how strongly the reward concentrates on the top of the judges' consensus. We train an open-weight Qwen3-4B Triage Agent within a fixed multi-agent Distributed Denial of Service (DDoS) alert-triage workflow on DARPA 2000 LLDOS 1.0 and test it on an independent CSE-CIC-IDS2018 DDoS trace. Across three training seeds, the agent reaches a mean F1-score of 0.869, 5.9 and 9.7 points above uniform insight weights and DIVA, and a false-positive rate of 4.9% versus 16.4% for GPT-5-mini. Within the weighting family, false positives fall only at the highest-orness weighting evaluated. All claims are limited to DDoS alert triage; the code, task contexts, and ranked insight dataset will be released.

==> Sections/Acknowledgements.tex <==
\section*{LLM usage}
This paper was edited for grammar using Grammarly and Claude.

==> Sections/Story.tex <==
% This file is dedicated to the story of the research
%we wanted to perform an RL workflow in the domain of DDOS attacks
We wanted to privatize and enhance an existing workflow for alert triaging in the cyber security.

\subsection{yossi workflow (with our small adjustments)}

first we searched what agent to optimize, out of the following

Context Gathering Agent:
This agent initiates the workflow. It takes the initial alert provided by the user and focuses on gathering the required preliminary context from the environment to set the stage for the investigation.

Triage Agent (Our Target Model):
Operating as the core investigative brain, this agent looks over the gathered context and decides the following course of actions :
\textbf{option 1:}
It generates specific forensic questions to uncover more details about the alert.

\textbf{option 2:}
If it determines there is enough evidence, it concludes the investigation by providing a final reasoning, an attack confidence score, and an impact score.

Question Answering Agent:
Whenever the Triage Agent asks a forensic question, this agent steps in. It executes the necessary tools or environmental queries to find the precise answer to the Triage Agent's question, passing the findings back so the Triage Agent can update its understanding.

Critique Agent:
When the Triage Agent decides to conclude the investigation with a final verdict and scoring, the Critique Agent acts as a safety validator.
It evaluates the reasoning and the evidence gathered. If the conclusion is found lacking or unsubstantiated, the Critique Agent rejects it, forcing the Triage Agent back into the questioning loop to gather more evidence.


The Workflow Connection:
The workflow resembles a continuous feedback loop. It begins with the Context Gathering Agent passing the initial intel to the Triage Agent, such intel is made by viewing the raised Suricata alerts.

The Triage Agent then cycles back and forth with the Question Answering Agent, iteratively asking questions to gather more evidence about the nature of the case and receiving answers.
Once the Triage Agent is confident enough to issue a final verdict, it submits its conclusion to the Critique Agent.
If approved, the workflow finishes and a report is generated; otherwise, the Triage Agent resumes its questioning loop.

\section{motivation for the project}
The motivation for the project is as follows:

\textbf{First} we wanted to transform the agents from closed source to opensource, as in the field of cyber security, we do not want to give closed-source model access to our private data.
However, this causes the problem of deploying large models within our resources limit, thus making us favor smaller models.

\textbf{second} we want to optimize a small and specialized model on our private data, thus gaining advantage on models that are tailored to our problem domain. Our goal is that such a lightweight model can capture the high-value investigative behaviors that are usually associated with much larger frontier models.

\textbf{third} the attacks we care about (e.g. DDoS campaigns) are multi-stage. A single alert such as a network scan rarely reveals the whole picture, and the true nature of the attack only becomes clear after combining later evidence such as service exploitation and coordinated communication patterns. Good triage therefore requires multi-step investigative reasoning over a hidden, only partially observable forensic structure, rather than a one-shot classification, and SOC analysts must do this over large volumes of heterogeneous alerts.

\textbf{fourth} the central constraint of our setting is that running full rollouts of the workflow is prohibitively expensive, so whatever method we use to train the triaging agent, it has to work \emph{without} completing full rollouts. This rules out standard end-of-rollout RL, whose reward is in any case sparse and delayed.

\textbf{fifth} the real question --- and the one our evaluation is built around --- is therefore which rollout-free way of training the triaging agent works best on our problem. Several existing algorithm families are rollout-free and can be adapted to our setting, so we take them and train our agent with each of them to compare against our approach.

\textbf{sixth} each of these candidates has a weakness that motivates a better signal. Supervised imitation of the expert steps (SFT) needs labels for intermediate steps that do not exist and tends to harm the model's reasoning; preference-based distillation (dDPO) and reinforcement learning from AI feedback (dRLAIF) also avoid rollouts, but they rely on coarse or single-judge signals that are not tailored to forensic quality.

\textbf{seventh} we are therefore motivated to design a rollout-free training signal built specifically for triage: a dense reward over the intermediate insights the agent produces, grounded in high-value insights proposed by a panel of SOTA models and organized into an \ac{I2C} so that no single judge's bias dominates. Our evaluation then compares this proposed reward head-to-head against SFT, dDPO, and dRLAIF on the same small base model.


\subsection{what we did}

Therefore, we wanted to decide what next steps we want to take in order to optimize the workflow.
We observed each agent behavior and how they operate with each other.
We realized that the workflow's investigative direction is usually defined by the triaging agent.

When starting the project, we knew that running complete rollouts of this workflow is highly expensive.
We were provided with $\sim$200 already existing alert investigations taken from the DARPA 2000 dataset that were conducted by GPT-5 mini.


% \subsection{first attempts}

% In order to improve the model as quickly as possible in the cheapest way (can utilize the investigations we already made) we first tried to take the triaging agent and perform SFT (distillation), for the qwen3 4b using the triaging steps the gpt 5 mini did in the already existing investigations.

% This indeed help us increase the performance - mostly in terms of precision, however we had the problem where the model's reasoning was greatly harmed.
% Therefore we wanted to see another approach such as RL, a big advantage of RL is that it lets the model adjust it's reasoning according to experiencing and not "disconnected training" such as supervised fine tuning.

\subsection{our solution}

We checked different algorithms such as Monte Carlo etc.; however, running full rollouts of the system is very expensive, and our domain problem is complex.

So we had to think of a way to give rewards to the investigative steps without completing full rollout.
Therefore, we attempted to think what defines a good question? Our answer is that it is something interesting to learn about the case given the context and that it relies on strong evidence from the context.

So we chose to define insights as things the llm generated to lead to its question that was inferred by the context.

Now we had to score insights with numerical reward. But as giving a strict grade to an investigation lead/step without full rollout is a hard task, we want to reduce it to another task which is more intuitive for an llm.

We paused our existing investigations at each time the triaging agent needs to speak.
To avoid continuing the workflow after each Triage Agent turn, we aimed to extract high-quality insights about the investigation and use RL to optimize our agent to produce as many high-quality insights as possible.

Practically, we asked a panel of SOTA models to look at that exact context and make their alternative triaging step.
Later we extracted the forensic insights they used from their answer and the context we gave them, the intuition for this being that we want our small model to make as many high quality SOTA insights.

But now we are left with the challenge: how do we grade each insight? We first attempted to use llm as a judge to grade the insights made by the experts so when our model makes them we know how to reward it (a failed attempt).

So we decided to do something else: compare and rank the insights to form an \ac{I2C}. Using a panel of SOTA models and comparative ranking, rather than a single model's absolute score, also mitigates the reward bias that comes from a single model self-evaluating its own insights.

So we use an LLM as a judge to order the \ac{I2C} entries from most critical (e.g., an encoded PowerShell command) to least critical (e.g., an odd timestamp).

